Fast 3D Extended Target Tracking using NURBS Surfaces

This paper proposes fast and novel methods to jointly estimate the target's unknown 3D shape and dynamics. Measurements are noisy and sparsely distributed 3D points from a light detection and ranging (LiDAR) sensor. The methods utilize non-uniform rational B-splines (NURBS) surfaces to approximate the target's shape. One method estimates Cartesian scaling parameters of a NURBS surface, whereas the second method estimates the corresponding NURBS weights, too. Major advantages are the capability of estimating a fully 3D shape as well as the fast processing time. Real-world evaluations with a static and dynamic vehicle show promising results compared to state-of-the-art 3D extended target tracking algorithms.

==> ass.tex <==
%\section{Augmented State Space} \label{sec:ass}
%
%\subsection{Measurement Model}
%%Boundary shape funciton: signed mahalonobis distance!
%
%
%\subsection{Motion Model}
%
%\begin{itemize}
%	\item Ackermann oder ACT
%	\item shape part is constant+noise
%\end{itemize}
%
%%\subsection{Inference}
%% Z_t = 0 0 0 0 0
%\begin{align}
%%\bm{Y}_t &= \begin{pmatrix} \bm{y}_{t1}^T,\dots,\bm{y}_{tn_t}^T  \end{pmatrix},\
%\bm{R}_t &= diag\begin{pmatrix} \bm{R}_{t1}^T,\dots,\bm{R}_{tn_t}^T  \end{pmatrix},\\
%\bm{h}\left(\bm{x}_t,\bm{Y}_{t},\bm{v}_t \right) &= \begin{pmatrix} h(\bm{x}_t,\bm{y}_{t1},\bm{v}_t)^T,\dots,h(\bm{x}_t,\bm{y}_{tn_t},\bm{v}_t)^T  \end{pmatrix}.
%\end{align}
%
%
%
%\begin{itemize}
%	\item sample based filter
%\end{itemize}
%
%

